The power disaggregation algorithms and their applications to demand dispatch

We were interested in solving a power disaggregation problem which comes down to estimating the power consumption of each device given the total power consumption of the whole house. We started by looking at the Factorial Hierarchical Dirichlet Process - Hidden Semi-Markov Model. However, the inference method had a complexity which scales withthe number of observations. Thus, we developed an online algorithm based on particle filters. We applied the method to data from Pecan Street https://dataport.cloud/ using Python. We applied the disaggregation algorithm to the control techniques used in Demand Dispatch.

==> Disaggregation.tex <==

\part{Disaggregation Problem}\label{disaggregation}

\include{Disaggregation/Model}

\include{Disaggregation/Inference}

\chapter{Applications}

